BreizhCrops: A Time Series Dataset for Crop Type Mapping

We present Breizhcrops, a novel benchmark dataset for the supervised classification of field crops from satellite time series. We aggregated label data and Sentinel-2 top-of-atmosphere as well as bottom-of-atmosphere time series in the region of Brittany (Breizh in local language), north-east France. We compare seven recently proposed deep neural networks along with a Random Forest baseline. The dataset, model (re-)implementations and pre-trained model weights are available at the associated GitHub repository (https://github.com/dl4sits/BreizhCrops) that has been designed with applicability for practitioners in mind. We plan to maintain the repository with additional data and welcome contributions of novel methods to build a state-of-the-art benchmark on methods for crop type mapping.

==> hyperparameter_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{rrr}
    \hline\
    \textbf{Models} & \textbf{Ranges} & \textbf{Selected value} \\
    \hline\hline
    
     \multicolumn{2}{l}{\textbf{TempCNN}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $2.38 \cdot 10^{-4}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $ 5.18 \cdot 10^{-5}$  \\
     Dropout rate & $\sim \mathcal{U}([0,0.8])$ & 0.18~\%\\
     Kernel sizes $K$ & $\{3,5,7\}$ & 7 \\
     Hidden units $H$ & $\{2^5,2^6,2^7\}$ & 128 \\
     %-- Cascaded layers $L$ & \multicolumn{2}{r}{3}\\
     No. runs & \multicolumn{2}{r}{78}  \\
     No. epochs & \multicolumn{2}{r}{11}  \\
     \hline
     
     \multicolumn{2}{l}{\textbf{MS-ResNet}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $6.27 \cdot 10^{-7}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $4.75 \cdot 10^{-6}$  \\
     Hidden units $H$ & $\{2^5,2^6,2^7,2^8,2^9\}$ & 32 \\
     No. runs & \multicolumn{2}{r}{70}  \\
     No. epochs & \multicolumn{2}{r}{23}  \\
     \hline
     
     \multicolumn{2}{l}{\textbf{InceptionTime}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $8.96 \cdot 10^{-3}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $2.22 \cdot 10^{-6}$  \\
     Hidden units $H$ & $\{2^5,2^6,2^7\}$ & 128 \\
     Cascaded layers $L$ & $\{1,2,3,4\}$ & 3\\
     No. runs & \multicolumn{2}{r}{86}  \\
     No. epochs & \multicolumn{2}{r}{23}  \\
     
     \hline
     \multicolumn{2}{l}{\textbf{OminiScale}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $1.06 \cdot 10^{-3}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $2.25 \cdot 10^{-7}$  \\
     No. runs & \multicolumn{2}{r}{39}  \\
     No. epochs & \multicolumn{2}{r}{19}  \\
     \hline\hline
     
     \multicolumn{2}{l}{\textbf{LSTM}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $9.88 \cdot 10^{-3}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $5.26 \cdot 10^{-7}$  \\
     Dropout rate & $\sim \mathcal{U}([0,0.8])$ & 0.57~\%\\
     Bidirectional & & \\
     Hidden units $H$ & $\{2^5,2^6,2^7\}$ & 128 \\
     Cascaded layers $L$ & $\{1,2,3,4\}$ & 3\\
     No. runs & \multicolumn{2}{r}{80}  \\
     No. epochs & \multicolumn{2}{r}{17}  \\
     
     \hline
     \multicolumn{2}{l}{\textbf{StarRNN}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $8.96 \cdot 10^{-3}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $ 2.22 \cdot 10^{-6}$  \\
     Dropout rate & $\sim \mathcal{U}([0,0.8])$ & 0.18~\%\\
     Hidden units $H$ & $\{2^5,2^6,2^7\}$ & 128 \\
     Cascaded layers $L$ & $\{1,2,3,4\}$ & 3\\
     No. runs & \multicolumn{2}{r}{84}  \\
     No. epochs & \multicolumn{2}{r}{17}  \\
     
     \hline\hline
     \multicolumn{2}{l}{\textbf{Transformer}} \\
     Learning rate $\nu$ & $\sim \mathcal{U}_\text{log}([10^{-2},10^{-4}])$ &  $1.31 \cdot 10^{-3}$ \\
     Weight decay $\lambda$ & $\sim \mathcal{U}_\text{log}([10^{-2}, 10^{-8}])$ & $5.52 \cdot 10^{-6}$  \\
     Dropout rate & $\sim \mathcal{U}([0,0.8])$ & 0.40~\%\\
     Self-attention head  & $\{1,2,3,4,5,6,7,8\}$ & 1 \\
     $N_{head}$ & &\\
     Hidden units $H$ & $\{2^5,2^6,2^7,2^8,2^9\}$ & 64 \\
     Cascaded layers $L$ & $\{1,2,3,4,5,6,7,8\}$ & 3\\
     No. runs & \multicolumn{2}{r}{39}  \\
     No. epochs & \multicolumn{2}{r}{26}  \\
     
     
     \hline\hline
\end{tabular}
\caption{Charlotte's test}
\label{tab:hyperparameter_values}
\end{table}
